Bulk and film synthesis pathways to ternary magnesium tungsten nitrides

Bulk solid state synthesis of nitride materials usually leads to thermodynamically stable, cation-ordered crystal structures, whereas thin film synthesis tends to favor disordered, metastable phases. This dichotomy is inconvenient both for basic materials discovery, where non-equilibrium thin film synthesis methods can be useful to overcome reaction kinetic barriers, and for practical technology applications where stable ground state structures are sometimes required. Here, we explore the uncharted Mg-W-N chemical phase space, using rapid thermal annealing to reconcile the differences between thin film and bulk powder syntheses. Combinatorial co-sputtering synthesis from Mg and W targets in a N$_2$ environment yielded cation-disordered Mg-W-N phases in the rocksalt (0.1< Mg/(Mg+W) <0.9), and hexagonal boron nitride (0.7< Mg/(Mg+W) <0.9) structure types. In contrast, bulk synthesis produced a cation-ordered polymorph of MgWN$_2$ that consists of alternating layers of rocksalt-like [MgN$_6$] octahedra and nickeline-like [WN$_6$] trigonal prisms (denoted "rocksaline"). Thermodynamic calculations corroborate these observations, showing rocksaline MgWN$_2$ is stable while other polymorphs are metastable. We also show that rapid thermal annealing can convert disordered rocksalt films to this cation-ordered polymorph near the MgWN$_2$ stoichiometry. Electronic structure calculations suggest that this rocksalt-to-rocksaline structural transformation should also drive a metallic-to-semiconductor transformation. In addition to revealing three new phases (rocksalt MgWN$_2$ and Mg$_3$WN$_4$, hexagonal boron nitride Mg$_3$WN$_4$, and rocksaline MgWN$_2$), these findings highlight how rapid thermal annealing can control polymorphic transformations, adding a new strategy for exploration of thermodynamic stability in uncharted phase spaces.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
